On the feasibility of dependency parsing of non-human sequences without a gold standard. Is evaluation possible in other species?

Dependency parsing consists of finding a tree representation for a sequence. Unsupervised dependency parsing aims to develop parsing methods without a gold standard during model training. In human languages, an unsupervised parser can be evaluated because some gold standard is usually available or can be created. For other species, a gold standard is unknown. Thus one may conclude that it is impossible to determine the accuracy of an unsupervised parser and, consequently, dependency parsing is unfeasible in other species. However, here we apply recent advances in network science to demonstrate that the proportion of correct edges retrieved by a parser must be high for the sequences of vocalizations or gestures that non-human primates produce due to the fast decay of the sequence length distribution. In contrast, human language sequences lack that property. Therefore, evaluation without a gold standard is feasible in non-human primates but a hard problem in humans.

==> table_of_contents.tex <==
\makeatletter
\newcommand{\mytableofcontents}{%
  \section*{Table of Contents}% Title of the TOC
  \@starttoc{toc}% Pulls data from the .toc file
}
\makeatother

% Fix clv2025 appendix referencing and add full titles to Table of Contents
\makeatletter
\let\oldappendixsection\appendixsection
\renewcommand{\appendixsection}[1]{%
  \oldappendixsection{#1}%
  \phantomsection
  \edef\@currentlabel{\thesection}%
  \addcontentsline{toc}{section}{Appendix \thesection: #1}%
}
\makeatother

\setcounter{tocdepth}{2} % Ensures subsections (depth 2) are rendered in the TOC

